CodexDB: Generating Code for Processing SQL Queries using GPT-3 Codex

CodexDB is an SQL processing engine whose internals can be customized via natural language instructions. CodexDB is based on OpenAI's GPT-3 Codex model which translates text into code. It is a framework on top of GPT-3 Codex that decomposes complex SQL queries into a series of simple processing steps, described in natural language. Processing steps are enriched with user-provided instructions and descriptions of database properties. Codex translates the resulting text into query processing code. An early prototype of CodexDB is able to generate correct code for a majority of queries of the WikiSQL benchmark and can be customized in various ways.

==> old/experiments.tex <==
\section{Experiments}
\label{sec:experiments}

t2.xlarge 

\begin{figure}[t]
    \centering
        \begin{tikzpicture}
        \begin{groupplot}[group style={group size=1 by 2, ylabels at=edge left, xlabels at=edge bottom}, width=8cm, height=3.5cm, legend entries={Question, Query, Plan}, legend columns=3, ymode=normal, ymajorgrids, xlabel={Number of samples}, ylabel={Nr.\ Solved}, legend to name=plainLegend, ylabel near ticks, xlabel near ticks, xtick={0, 2, 4}, ybar, nodes near coords, enlargelimits=0.275]
        \nextgroupplot[title=Cushman-Codex Model]
        \addplot coordinates {(0, 0) (2, 81) (4, 19)};
        \addplot coordinates {(0, 0) (2, 78) (4, 21)};
        \addplot coordinates {(0, 69) (2, 89) (4, 0)};
            
        \nextgroupplot[title=Davinci-Codex Model]
        \addplot coordinates {(0, 0) (2, 83) (4, 84)};
        \addplot coordinates {(0, 0) (2, 80) (4, 84)};
        \addplot coordinates {(0, 79) (2, 91) (4, 90)};
        \end{groupplot}    
    \end{tikzpicture}
    
    \ref{plainLegend}
    \caption{Number of test cases solved out of 100 with modification ``use pandas library''.}
    \label{fig:pandas}
\end{figure}

%Median generation time 3 seconds for Cushman (0-shot) and 6 for Davinci. (2-shot: 5; 12. 4-shot: 13 for Davinci (none solved for Cushman); 

3 seconds median generation time for Cushman, 12 for Davinci

Training took 492 seconds, 42 out of 50 test cases solved, median of 1 try per case and average of 2.66 tries per test case.

\begin{figure}[t]
    \centering
        \begin{tikzpicture}
        \begin{groupplot}[group style={group size=1 by 2, ylabels at=edge left, x descriptions at=edge bottom}, width=8.25cm, height=3.5cm, legend entries={SQL Engine, Generated Code}, legend columns=2, ymode=normal, ymajorgrids, xlabel={Queries}, xtick=\empty, ylabel={Time (s)}, legend to name=plainLegend, ylabel near ticks, xlabel near ticks, ybar, xmin=0, xmax=26, ymode=log]
        \nextgroupplot[title={Scaling Factor 1,000}, bar width=1.75px]
        \addplot table[col sep=comma, x expr={\pgfplotstablerow+1}, y index=1, skip first n=1] {plots/performance/sql/times_25.csv};
        \addplot table[col sep=comma, x expr={\pgfplotstablerow+1}, y index=1, skip first n=1] {plots/performance/pandas/times_25.csv};
        
        \nextgroupplot[title={Scaling Factor 100,000}, bar width=1.75px]
        \addplot table[col sep=comma, x expr={\pgfplotstablerow+1}, y index=2, skip first n=1] {plots/performance/sql/times_25.csv};
        \addplot table[col sep=comma, x expr={\pgfplotstablerow+1}, y index=2, skip first n=1] {plots/performance/pandas/times_25.csv};
        \end{groupplot}
    \end{tikzpicture}
    
    \ref{plainLegend}
    \caption{Performance evaluation of generated code.}
    \label{fig:performance}
\end{figure}

\begin{figure}[t]
    \centering
        \begin{tikzpicture}
        \begin{groupplot}[group style={group size=1 by 2, ylabels at=edge left, xlabels at=edge bottom}, width=8cm, height=3.5cm, legend entries={pandas,vaex,parallel,pandas+completed,pandas+results,pandas+progress}, legend columns=3, ymode=normal, ymajorgrids, xlabel={Number of samples}, ylabel={Nr.\ Solved}, legend to name=plainLegend, ylabel near ticks, xlabel near ticks, xtick={0, 2, 4}, ybar, nodes near coords, enlargelimits=0.275]
        \nextgroupplot[title=Cushman-Codex Model, bar width=7px]
        \addplot coordinates {(0, 69) (2, 89) (4, 0)};
        \addplot coordinates {(0, 2) (2, 64) (4, 0)};
        \addplot coordinates {(0, 12) (2, 71) (4, 0)};
        \addplot coordinates {(0, 44) (2, 41) (4, 0)};
        \addplot coordinates {(0, 52) (2, 2) (4, 0)};
        \addplot coordinates {(0, 37) (2, 37) (4, 0)};

        \nextgroupplot[title=Davinci-Codex Model, bar width=7px]
        \addplot coordinates {(0, 79) (2, 91) (4, 90)};
        \addplot coordinates {(0, 5) (2, 58) (4, 60)};
        \addplot coordinates {(0, 11) (2, 68) (4, 59)};
        \addplot coordinates {(0, 25) (2, 66) (4, 64)};
        \addplot coordinates {(0, 57) (2, 56) (4, 59)};
        \addplot coordinates {(0, 20) (2, 71) (4, 69)};
        \end{groupplot}
    \end{tikzpicture}
    
    \ref{plainLegend}
    \caption{Number of test cases solved out of 100 for different modifications.}
    \label{fig:modifications}
\end{figure}

\begin{table}
    \centering
    \caption{Code length in characters for different language and modifications.}
    \begin{tabular}{lp{3.25cm}lll}
    \toprule[1pt]
         Language & Modification & Min & Median & Max \\
    \midrule[1pt]
         SQL & - & 42 & 77 & 227 \\
         \midrule
         Python & use pandas library & 548 & 1117 & 1607 \\
         \midrule
         & use vaex library & 860 & 1710 & 2126 \\
         \midrule
         & use parallel processing & 904 & 1738 & 2430 \\
         \midrule
         & use pandas library; print out 'Step completed!' & 759 & 1567 & 2566 \\
         \midrule
         & use pandas library; print out intermediate result & 992 & 1860 & 2352 \\
         \midrule
         & use pandas library; print progress updates & 1000 & 1934 & 2483 \\
         \bottomrule 
    \end{tabular}
    \label{tab:codesize}
\end{table}

Pandas version: execution times between 0.46 and 0.52 seconds (median is 0.48 seconds).


==> sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
